Calibration of Neural Networks using Splines

Calibrating neural networks is of utmost importance when employing them in safety-critical applications where the downstream decision making depends on the predicted probabilities. Measuring calibration error amounts to comparing two empirical distributions. In this work, we introduce a binning-free calibration measure inspired by the classical Kolmogorov-Smirnov (KS) statistical test in which the main idea is to compare the respective cumulative probability distributions. From this, by approximating the empirical cumulative distribution using a differentiable function via splines, we obtain a recalibration function, which maps the network outputs to actual (calibrated) class assignment probabilities. The spine-fitting is performed using a held-out calibration set and the obtained recalibration function is evaluated on an unseen test set. We tested our method against existing calibration approaches on various image classification datasets and our spline-based recalibration approach consistently outperforms existing methods on KS error as well as other commonly used calibration measures. Our Code is available at https://github.com/kartikgupta-at-anu/spline-calibration.

==> newcommands.tex <==
\newcommand{\IO}{{[ \m I \mid \vs 0 ]}}
\newcommand{\Rc}{{[ \m R \mid -\m R \dH C ]}}
\newcommand{\alg} {{\mbox{\rm\small alg}}}
\newcommand{\sym} {{\mbox{\rm\small sym}}}
\newcommand{\barH}{{\bar{\m H}}}
\newcommand{\barN}{{\bar{\vs N}}}
\newcommand{\barX}{{\bar{\vs X}}}
\newcommand{\barh}{{\bar{\v h}}}
\newcommand{\barm}{{\bar{\v m}}}
\newcommand{\barp}{{\bar{\v p}}}
\newcommand{\barv}{{\bar{\v v}}}
\newcommand{\barx}{{\bar{\v x}}}
\newcommand{\cam}{{\mbox{\rm\small cam}}}
\newcommand{\dH}[1]{{\tilde{\vs #1}}}
\newcommand{\depth}{\mbox{\rm depth}}
\newcommand{\Dh}[1]{{\tilde{\v #1}}}
\newcommand{\geom}{{\mbox{\rm\small geom}}}
\newcommand{\mah}{{\mbox{\rm\small Mah}}}
\newcommand{\hath}{{\hat{\v h}}}
\newcommand{\hatf}{{\hat{\v f}}}
\newcommand{\hatH}{{\widehat{\m H}}}
\newcommand{\hatA}{{\widehat{\m A}}}
\newcommand{\hatN}{{\hat{\vs N}}}
\newcommand{\hatX}{{\widehat{\vs X}}}
\newcommand{\hatm}{{\hat{\v m}}}
\newcommand{\hatp}{{\hat{\v p}}}
\newcommand{\hatu}{{\hat{\v u}}}
\newcommand{\hatx}{{\hat{\v x}}}
\newcommand{\haty}{{\hat{\v y}}}
\newcommand{\hatvP}{{\widehat{\vs P}}}
\newcommand{\hatP}{{\widehat{\m P}}}
\newcommand{\hatF}{{\widehat{\m F}}}
\newcommand{\lin}[2]{<#1; #2>}
\newcommand{\matxs}[1]{{\tt  \tilde{#1}}}
\newcommand{\pqrs}{^{pqrs}}
\newcommand{\tens}[2]{#1_{#2}}
\newcommand{\tilA}{{\widetilde{\m A}}}
\newcommand{\tilC}{{\widetilde{\vs C}}}
\newcommand{\tilH}{{\widetilde{\m H}}}
\newcommand{\tilx}{{\tilde{\v x}}}
\newcommand{\tilh}{{\tilde{\v h}}}
\newcommand{\x}{{\mbox{\sl\sc x}}}
\newcommand{\y}{{\mbox{\sl\sc y}}}
\newcommand{\z}{{\mbox{\sl\sc z}}}
\newcommand{\T}{{\mbox{\sl\sc t}}}
\newcommand{\X}{{\mbox{\sl\sc x}}}
\newcommand{\Y}{{\mbox{\sl\sc y}}}
\newcommand{\Z}{{\mbox{\sl\sc z}}}
\newcommand{\W}{{\mbox{\sl\sc w}}}
%
% for subscripts/superscripts for affine and projective H's etc
%
\newcommand{\HE}{{\rm E}}
\newcommand{\HM}{{\rm M}}
\newcommand{\HS}{{\rm S}}
\newcommand{\HA}{{\rm A}}
\newcommand{\HP}{{\rm P}}

% \newcommand{\symm}{{\mbox{\small S}}}
% \newcommand{\anti}{{\mbox{\small A}}}
% would prefer to have these symbols with small upper case
% but caption lines then too long
\newcommand{\symm}{{\mbox{\tt s}}}
\newcommand{\anti}{{\mbox{\tt a}}}
\newcommand{\ray}[2]{\overline{#1 #2}}

% The calibration matrix -- Andrew, we can not use $\m C$, since
% this is used (in close proximity) as the symbol for a conic.
\newcommand{\K}{\m K}

% Temporarily like this to satisfy version of latex
%\newcommand{\x}{X}
%\newcommand{\y}{Y}
%\newcommand{\z}{Z}
%\newcommand{\T}{T}
%\newcommand{\X}{X}
%\newcommand{\Y}{Y}
%\newcommand{\Z}{Z}
%\newcommand{\W}{W}

% For the image of X under the Carlsson map
\newcommand{\invX}{{\bar{\vs X}}}
\newcommand{\barC}{{\bar{\vs C}}}
\newcommand{\invC}{{\bar{\vs C}}}
\newcommand{\barQ}{{\bar{\m Q}}}
\newcommand{\barP}{{\bar{\m P}}}
\newcommand{\barF}{{\bar{\m F}}}


==> theorenv.tex <==
%
% Derived from article.sty and eccv92.sty
%

\catcode`\@=11

%
%
% New theorem environments
%
%
\newif\if@envcountreset\@envcountresetfalse
\def\ds@envcountreset{\@envcountresettrue}
\def\ts{\thinspace}
%
% new environments and theorems
% borrowed form the LTMP-style of Springer-Verlag
% designed by Dr. Christoph Ender
%
% define the new theorem like environments
% define a new style of environments where it is possible to define
% the font % used as the theorem name and the fontfamily for the text.
%
% \newstytheorem{name}{thefont}{txtfont}{Text}[Counter]
% \newstytheorem{name}{thefont}{txtfont}[oldname]{Text}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
%
\def\newstytheorem#1#2#3{%
\@ifnextchar[{\che@othm{#1}{#2}{#3}}{\che@nthm{#1}{#2}{#3}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
%
\def\che@nthm#1#2#3#4{%
\@ifnextchar[{\che@xnthm{#1}{#2}{#3}{#4}}{\che@ynthm{#1}{#2}{#3}{#4}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
% #5 - add theorem counter to reset list of another counter
%
\def\che@xnthm#1#2#3#4[#5]{\expandafter
\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}\if@envcountreset\@addtoreset{#1}{#5}\fi
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\che@thm{#1}{#4}{#2}{#3}}\global
\@namedef{end#1}{\@endtheorem}}}
%
% #1 - name of theorem
% #2 - theorem font
% #3 - text font
% #4 - text string of thorem name
%
\def\che@ynthm#1#2#3#4{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\che@thm{#1}{#2}{#3}{#4}}\global
\@namedef{end#1}{\@endtheorem}}}
%
% change oldthm if oldname in specification is '*'
% then don't use a counter
% #1 - countername
% #2 - theorem font
% #3 - text font
% #4 - counter used
% #5 - string containing theorem name to print
%
\def\che@othm#1#2#3[#4]#5{\expandafter\@ifdefinable
\csname#1\endcsname%
{\@@othm@{#1}{#2}{#3}{#4}{#5}\global\@namedef{end#1}{\@endtheorem}}}
%
\def\@@othm@#1#2#3#4#5{\if *#4{\global\@namedef{the#1}{\relax}
\global\@namedef{#1}{\@bthm@{}{#5}{#2}{#3}}}\else
{\global\@namedef{the#1}{\@nameuse{the#4}}% define the counter
\global\@namedef{#1}{\che@thm{#4}{#5}{#2}{#3}}}\fi}
%
% new defs for theorem environment che 17-MAR-1989
% it improves the option possible
%
% #1 - countername  = theorem name
% #2 - string containing theorem name to print
% #3 - theorem font
% #4 - text font
\def\che@thm#1#2#3#4{\@ifnextchar({\@athm{#1}{#2}{#3}{#4}}{%
\@ifnextchar *{\@bthm{#1}{#2}{#3}{#4}}%
{\@@thm{#1}{#2}{#3}{#4}}}}
%
% \begin{thm}(A.1)[test]      results in:
% \end{thm}                               thm A.1 (test) ....
% #1 - theorem
% #2 - string of theorem name
% #3 - font for theorem name and label
% #4 - Text font
% #5 - is the new label
% #6 - optional string
%
\def\@athm#1#2#3#4(#5){\@ifnextchar[{%
\@aythm{#1}{#2}{#3}{#4}{#5}}{\@axthm{#1}{#2}{#3}{#4}{#5}}}
\def\@axthm#1#2#3#4#5{\@@locthmlab{#1}{#5}%
\@begintheorem{#2}{#5}{#3}{#4}\ignorespaces}
\def\@aythm#1#2#3#4#5[#6]{\@@locthmlab{#1}{#5}%
\fuh@opargbegintheorem{#2}{#5}{#6}{#3}{#4}\ignorespaces}
%
% \begin{thm}*[xytest]        results in:
% \end{thm}                               thm (xytest) ....
% #1 - theorem
% #2 - string of theorem name
% #3 - font for theorem name and label
% #4 - Text font
% #5 - optional string
%
\def\@bthm@#1#2#3#4{\@ifnextchar[{\@bythm{#1}{#2}{#3}{#4}}{%
\@bxthm{#1}{#2}{#3}{#4}}}
\def\@bthm#1#2#3#4*{\@ifnextchar[{\@bythm{#1}{#2}{#3}{#4}}{%
\@bxthm{#1}{#2}{#3}{#4}}}
\def\@bxthm#1#2#3#4{\if !#1!\relax\else\@@locthmlab{#1}{}\fi
\@@begintheorem{#2}{#3}{#4}\ignorespaces}
\def\@bythm#1#2#3#4[#5]{%
\@@opargbegintheorem{#2}{#3}{#4}{#5}\ignorespaces}
%
% define local label
%   if no number or a user specified label occured
%
\def\@@locthmlab#1#2{\expandafter\def\csname the#1\endcsname{#2}
\let\@chetempa\protect\def\protect{\noexpand\protect\noexpand}%
\edef\@currentlabel{\csname p@#1\endcsname\csname the#1\endcsname}%
\let\protect\@chetempa}
%
% #1 - counter = theorem name
% #2 - string with name
% #3 - font for theorem name and label
% #4 - font for text
\def\@@thm#1#2#3#4{\refstepcounter
    {#1}\@ifnextchar[{\che@ythm{#1}{#2}{#3}{#4}}{%
    \che@xthm{#1}{#2}{#3}{#4}}}
%
\def\che@xthm#1#2#3#4{\che@begintheorem{#2}{\csname
the#1\endcsname}{#3}{#4}\ignorespaces}
\def\che@ythm#1#2#3#4[#5]{\che@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#5}{#3}{#4}\ignorespaces}
%
% #1 - name of theorem
% #2 - label string
% #3 - font for name and lable
% #4 - text fomt
%
\def\che@begintheorem#1#2#3#4{#4\trivlist\item[#3 #1\ts #2.]}
%
% #1 - name of theorem
% #2 - label string
% #3 - additonal text
% #4 - font for name and lable
% #5 - text fomt
%
\def\che@opargbegintheorem#1#2#3#4#5{#5 \trivlist
\item[#4 #1\ts #2\ #3.]}
%
\def\fuh@opargbegintheorem#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3).}]}
%
\def\@@begintheorem#1#2#3{#3\trivlist\item[#2 #1.]}
\def\@@opargbegintheorem#1#2#3#4{#3\trivlist\item[#2 #1 #4.]}
 
\newstytheorem{theorem}{\bf}{\it}{Theorem}[section]
\newstytheorem{conjecture}{\bf}{\it}{Conjecture}[section]
\newstytheorem{example}{\bf}{\rm}[theorem]{Example}
\newstytheorem{proposition}{\bf}{\it}[theorem]{Proposition}
\newstytheorem{corollary}{\bf}{\it}[theorem]{Corollary}
\newstytheorem{lemma}{\bf}{\it}[theorem]{Lemma}
\newstytheorem{proof}{\it}{\rm}[*]{Proof}
\newstytheorem{definition}{\bf}{\rm}[theorem]{Definition}
\newstytheorem{remark}{\it}{\rm}[*]{Remark}
\newstytheorem{exercise}{\it}{\rm}[theorem]{Exercise}
\newstytheorem{problem}{\it}{\rm}[theorem]{Problem}
\newstytheorem{solution}{\it}{\rm}[theorem]{Solution}
\newstytheorem{note}{\it}{\rm}[theorem]{Note}
\newstytheorem{question}{\it}{\rm}[theorem]{Question}
\newstytheorem{condition}{\it}{\rm}[theorem]{Condition}
\newstytheorem{algorithm}{\bf}{\rm}[theorem]{Algorithm}
\newstytheorem{numbered}{\bf}{\it}[theorem]{}
\renewcommand{\thenumbered}{(\thesection.\arabic{numbered})}
%\newstytheorem{unnumbered}{\bf}{\it}[*]{~~~$\bullet$\hspace*{-18pt}~~~} 
\newenvironment{unnumbered}{\begin{itemize}\item\em}{\end{itemize}}
\renewcommand{\thetheorem}{\thesection.\arabic{theorem}}
 
% qed sign
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\catcode`\@=12

%\newstytheorem{unnumbered}{\bf}{\it}[*]{~~~$\bullet$\hspace*{-18pt}~~~} 
%\renewcommand{\thenumbered}{(\thechapter.\arabic{numbered})}


